Opportunistic hip fracture risk prediction in Men from X-ray: Findings from the Osteoporosis in Men (MrOS) Study

Osteoporosis is a common disease that increases fracture risk. Hip fractures, especially in elderly people, lead to increased morbidity, decreased quality of life and increased mortality. Being a silent disease before fracture, osteoporosis often remains undiagnosed and untreated. Areal bone mineral density (aBMD) assessed by dual-energy X-ray absorptiometry (DXA) is the gold-standard method for osteoporosis diagnosis and hence also for future fracture prediction (prognostic). However, the required special equipment is not broadly available everywhere, in particular not to patients in developing countries. We propose a deep learning classification model (FORM) that can directly predict hip fracture risk from either plain radiographs (X-ray) or 2D projection images of computed tomography (CT) data. Our method is fully automated and therefore well suited for opportunistic screening settings, identifying high risk patients in a broader population without additional screening. FORM was trained and evaluated on X-rays and CT projections from the Osteoporosis in Men (MrOS) study. 3108 X-rays (89 incident hip fractures) or 2150 CTs (80 incident hip fractures) with a 80/20 split were used. We show that FORM can correctly predict the 10-year hip fracture risk with a validation AUC of 81.44 +- 3.11% / 81.04 +- 5.54% (mean +- STD) including additional information like age, BMI, fall history and health background across a 5-fold cross validation on the X-ray and CT cohort, respectively. Our approach significantly (p < 0.01) outperforms previous methods like Cox Proportional-Hazards Model and \frax with 70.19 +- 6.58 and 74.72 +- 7.21 respectively on the X-ray cohort. Our model outperform on both cohorts hip aBMD based predictions. We are confident that FORM can contribute on improving osteoporosis diagnosis at an early stage.

==> MrOS Miccai/images.tex <==
\usepackage{caption}
\usepackage{subcaption}

\newcommand{\pic}[3]{
	\begin{figure}[tb] 
		\centering
		\includegraphics[width=#3\linewidth]{#1}
		\caption{#2}
		\label{fig:#1}
	\end{figure}
}

\newcommand{\picTwo}[4]{
	\begin{figure*}[tb]
		\centering
		\begin{subfigure}[c]{0.49\textwidth}
			\centering		
			\includegraphics[width=0.9\textwidth]{#1-0}
			\subcaption{#2}	
			\label{fig:#1-0}	
		\end{subfigure}
		\begin{subfigure}[c]{0.49\textwidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-1}
			\subcaption{#3}
			\label{fig:#1-1}	
		\end{subfigure}
		\caption{#4}
		\label{fig:#1}
	\end{figure*}
}

\newcommand{\picTwoAsym}[4]{
	\begin{figure*}[tb]
		\centering
		\begin{subfigure}[c]{0.64\textwidth}
			\centering		
			\includegraphics[width=0.9\textwidth]{#1-0}
			\subcaption{#2}	
			\label{fig:#1-0}	
		\end{subfigure}
		\begin{subfigure}[c]{0.35\textwidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-1}
			\subcaption{#3}
			\label{fig:#1-1}	
		\end{subfigure}
		\caption{#4}
		\label{fig:#1}
	\end{figure*}
}

\newcommand{\picThree}[5]{
	\begin{figure*}[tb]
		\centering
		\begin{subfigure}[c]{0.325\textwidth}
			\centering		
			\includegraphics[width=0.9\textwidth]{#1-0}
			\subcaption{#2}	
				\label{fig:#1-0}	
		\end{subfigure}
		\begin{subfigure}[c]{0.325\textwidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-1}
			\subcaption{#3}	
				\label{fig:#1-1}	
		\end{subfigure}
		\begin{subfigure}[c]{0.325\textwidth}	
			\centering	
			\includegraphics[width=0.9\textwidth]{#1-2}
			\subcaption{#4}	
				\label{fig:#1-2}	
		\end{subfigure}
	
		\caption{#5}
		\label{fig:#1}
	\end{figure*}
}

\newcommand{\picFour}[6]{
	\begin{figure*}[htb]
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#1-0}
				\subcaption{#2}	
				\label{fig:#1-0}
		\end{subfigure}
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#1-1}
				\subcaption{#3}	
				\label{fig:#1-1}
		\end{subfigure}
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#1-2}
				\subcaption{#4}	
				\label{fig:#1-2}
		\end{subfigure}
		\begin{subfigure}[c]{0.24\textwidth}		
			\includegraphics[width=\textwidth]{#1-3}
				\subcaption{#5}
				\label{fig:#1-3}
		\end{subfigure}	
		\caption{#6}
		\label{fig:#1}
	\end{figure*}
}


==> MrOS Miccai/tables.tex <==
\usepackage{tabularx}
\usepackage{multirow}
\usepackage{booktabs}  
\usepackage{colortbl}  
\definecolor{LightGray}{rgb}{0.95,0.95,0.95}

\newcommand{\tblStatistics}{
\begin{table}[tb]
		\caption{
		Statistics for three different cohorts (all, CT or X-Ray data available). 
		For each cohort we give the statistics for the complete cohort and with respect to the hip fracture horizon with (w) and without (w/o) fracture (fx).
		$n$ represents the number of samples. Age is given as relative percentage for a specific range from $n$. 
		Training / Validation refer to the number of used images in the respective sets in the first fold.
		 - means that no data was used for training or validation.
		All other risk factors are given as mean (STD in brackets).
	}
	\label{tbl:statistics}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{l c c c  c c c c c  c c c }
			& \multicolumn{3}{c}{Cohort All} & \multicolumn{5}{c}{Cohort CT} & \multicolumn{3}{c}{Cohort X-Ray}\\
			\cmidrule(r){2-4} \cmidrule(r){5-9} \cmidrule{10-12}
			
			& & \multicolumn{2}{c}{$t$ = 10 year} & & \multicolumn{2}{c}{$t$ = 10 year} & \multicolumn{2}{c}{$t$ = 5 year} & & \multicolumn{2}{c}{$t$ = 10 year} \\
			\cmidrule(r){3-4} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule{11-12}
			
			& all & w/o fx & w fx & all & w/o fx & w fx  & w/o fx & w fx & all & w/o fx & w fx \\
			
			\rowcolor{LightGray}
			
		    $n$ & 5994 & 4004 & 185 & 3165 & 2150 & 80 & 2198 & 32 & 3895 & 3108 & 89 \\
		    
		    Age [\%] \makecell{64-69\\70-74\\75-79\\80+} & \makecell{29.51\\28.50\\24.11\\17.88} & \makecell{36.69\\31.87\\21.98\\9.47} & \makecell{10.27\\16.22\\33.51\\40.00} 
 & \makecell{30.74\\28.44\\23.70\\17.12} & \makecell{37.86\\32.00\\21.44\\8.70} & \makecell{16.25\\15.00\\37.50\\31.25}  & \makecell{37.44\\31.71\\21.84\\9.01} & \makecell{12.50\\9.38\\34.38\\43.75}   & \makecell{32.99\\30.40\\23.90\\12.71} & \makecell{37.32\\31.66\\22.30\\8.72} & \makecell{15.73\\19.10\\39.33\\25.84}  \\ 
 
 \rowcolor{LightGray}
 
		      Height [m] & \makecell{1.74\\(0.07)}  & \makecell{1.75\\(0.07)}   & \makecell{1.73\\(0.06)}  & \makecell{1.74\\(0.07)}  & \makecell{1.75\\(0.07)}   & \makecell{1.74\\(0.06)}  & \makecell{1.75\\(0.07)}   & \makecell{1.72\\(0.06)}  & \makecell{ 1.74\\(0.07)}  & \makecell{1.74\\(0.07)}   & \makecell{1.74\\(0.06)}    \\

BMI [$\frac{kg}{m^2}$] & \makecell{25.90\\(3.65)}  & \makecell{26.00\\(3.54)}   & \makecell{25.11\\(3.63)}   & \makecell{25.80\\(3.60)}  & \makecell{25.89\\(3.48)}   & \makecell{24.77\\(3.38)}   & \makecell{ 25.86\\(3.49)}   & \makecell{24.68\\(3.02)}   & \makecell{25.86\\(3.57)}  & \makecell{25.90\\(3.48)}   & \makecell{24.86\\(3.65)}   \\

\midrule

\rowcolor{LightGray}

\makecell{Femoral aBMD\\$[\frac{g}{cm^2}]$}  & \makecell{0.78\\(0.13)}  & \makecell{0.79\\(0.13)}   & \makecell{0.66\\(0.11)}    & \makecell{0.78\\(0.13)}  & \makecell{0.79\\(0.13)}   & \makecell{0.65\\(0.08)}   & \makecell{0.79\\(0.13)}   & \makecell{0.62\\(0.08)}   & \makecell{ 0.79\\(0.13)}  & \makecell{0.79\\(0.12)}   & \makecell{0.68\\(0.10)}     \\



\makecell{Spine aBMD\\ $[\frac{g}{cm^2}]$} & \makecell{1.07\\(0.19)}  & \makecell{1.07\\(0.18)}   & \makecell{1.01\\(0.19)}   & \makecell{1.07\\(0.19)}  & \makecell{1.06\\(0.18)}   & \makecell{1.00\\(0.16)}   & \makecell{1.06\\(0.18)}   & \makecell{0.98\\(0.19)}  & \makecell{1.07\\(0.18)}  & \makecell{1.07\\(0.18)}   & \makecell{1.00\\(0.20)}   \\

\rowcolor{LightGray}

Avg. TBS & \makecell{1.23\\(0.13)}  & \makecell{1.23\\(0.13)}   & \makecell{1.19\\(0.13)}   & \makecell{ 1.23\\(0.13)}  & \makecell{1.24\\(0.12)}   & \makecell{1.20\\(0.12)}   & \makecell{1.24\\(0.12)}   & \makecell{1.17\\(0.13)}     & \makecell{1.24\\(0.12)}  & \makecell{1.24\\(0.12)}   & \makecell{1.19\\(0.12)}     \\



\frax [\%] & \makecell{4.14\\(4.39)}  & \makecell{3.14\\(3.07)}   & \makecell{7.04\\(5.67)}   & \makecell{4.01\\(4.28)}  & \makecell{3.04\\(2.93)}   & \makecell{6.29\\(5.85)}   & \makecell{3.07\\(2.94)}   & \makecell{8.53\\(7.97)}   & \makecell{3.54\\(3.56)}  & \makecell{3.07\\(2.89)}   & \makecell{5.76\\(4.87)}    \\

\rowcolor{LightGray}

\makecell{\frax (w. aBMD)\\ $ [\%] $ } & \makecell{ 4.45\\(5.54)}  & \makecell{3.38\\(4.04)}   & \makecell{10.86\\(9.09)}  & \makecell{4.33\\(5.41)}  & \makecell{3.35\\(3.95)}   & \makecell{10.47\\(8.92)}   & \makecell{  3.45\\(4.12)}   & \makecell{14.38\\(9.41)}  & \makecell{3.85\\(4.74)}  & \makecell{3.34\\(3.95)}   & \makecell{9.41\\(8.56)}     \\
		    
		    \midrule
		    
		     
			
	        Training & - & - & - & - & 3403 & 128 & 3478 & 53 & - & 4353 & 107 \\
	       \rowcolor{LightGray}
	        
	        Validation & - & - & - & - & 790 & 27 & 810 & 7 & - &  1086 & 35 \\
			
		\end{tabular}
	}


	
\end{table}
}



\newcommand{\tblDatasetsExtend}{
\begin{table}[tb]
		\caption{
		Dataset statistics --- TODO some falls values for 5 year ct
	}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{l c c c  c c c c c  c c c }
			& \multicolumn{3}{c}{Cohort All} & \multicolumn{5}{c}{Cohort CT} & \multicolumn{3}{c}{Cohort X-Ray}\\
			\cmidrule(r){2-4} \cmidrule(r){5-9} \cmidrule{10-12}
			
			& & \multicolumn{2}{c}{10 year} & & \multicolumn{2}{c}{10 year} & \multicolumn{2}{c}{5 year} & & \multicolumn{2}{c}{10 year} \\
			\cmidrule(r){3-4} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule{11-12}
			
			& all & w/o fx & w fx & all & w/o fx & w fx  & w/o fx & w fx & all & w/o fx & w fx \\
			
		    n & 5994 & 4004 & 185 & 3165 & 2150 & 80 & 2792 & 32 & 3895 & 3108 & 89 \\
		    Age [yrs] \makecell{64-69\\70-74\\75-79\\80+} & \makecell{29.51\\28.50\\24.11\\17.88} & \makecell{36.69\\31.87\\21.98\\9.47} & \makecell{10.27\\16.22\\33.51\\40.00} 
 & \makecell{30.74\\28.44\\23.70\\17.12} & \makecell{37.86\\32.00\\21.44\\8.70} & \makecell{16.25\\15.00\\37.50\\31.25}  & \makecell{32.88\\29.84\\23.57\\13.72} & \makecell{12.50\\9.38\\34.38\\43.75}  & \makecell{32.99\\30.40\\23.90\\12.71} & \makecell{37.32\\31.66\\22.30\\8.72} & \makecell{15.73\\19.10\\39.33\\25.84}  \\ 
		    Height [m] & 1.74 $\pm$ 0.07 [1.47 - 1.99] & 1.75 $\pm$ 0.07 [1.52 - 1.99]  & 1.73 $\pm$ 0.06 [1.58 - 1.91] & 1.74 $\pm$ 0.07 [1.47 - 1.99] & 1.75 $\pm$ 0.07 [1.52 - 1.99]  & 1.74 $\pm$ 0.06 [1.64 - 1.91] & 1.74 $\pm$ 0.07 [1.52 - 1.99]  & 1.72 $\pm$ 0.06 [1.64 - 1.85] &  1.74 $\pm$ 0.07 [1.52 - 1.98] & 1.74 $\pm$ 0.07 [1.52 - 1.98]  & 1.74 $\pm$ 0.06 [1.59 - 1.89]   \\
		    
		    BMI [$\frac{kg}{m^2}$] & 25.90 $\pm$ 3.65 [15.72 - 48.52] & 26.00 $\pm$ 3.54 [16.85 - 48.52]  & 25.11 $\pm$ 3.63 [18.23 - 35.74]  & 25.80 $\pm$ 3.60 [15.72 - 44.79] & 25.89 $\pm$ 3.48 [17.24 - 40.08]  & 24.77 $\pm$ 3.38 [19.22 - 35.59]  &  25.84 $\pm$ 3.57 [15.72 - 44.79]  & 24.68 $\pm$ 3.02 [20.07 - 35.59]  & 25.86 $\pm$ 3.57 [16.32 - 48.52] & 25.90 $\pm$ 3.48 [16.85 - 48.52]  & 24.86 $\pm$ 3.65 [18.23 - 35.59]  \\
		    
		    \midrule
		    
		    Femoral aBMD [$\frac{g}{cm^2}$]  & 0.78 $\pm$ 0.13 [0.27 - 1.60] & 0.79 $\pm$ 0.13 [0.44 - 1.60]  & 0.66 $\pm$ 0.11 [0.27 - 0.97]   & 0.78 $\pm$ 0.13 [0.35 - 1.49] & 0.79 $\pm$ 0.13 [0.44 - 1.49]  & 0.65 $\pm$ 0.08 [0.45 - 0.87]  & 0.79 $\pm$ 0.13 [0.35 - 1.49]  & 0.62 $\pm$ 0.08 [0.49 - 0.87]  &  0.79 $\pm$ 0.13 [0.35 - 1.49] & 0.79 $\pm$ 0.12 [0.44 - 1.49]  & 0.68 $\pm$ 0.10 [0.45 - 0.97]    \\
		    Spine aBMD [$\frac{g}{cm^2}$] & 1.07 $\pm$ 0.19 [0.47 - 2.10] & 1.07 $\pm$ 0.18 [0.49 - 1.99]  & 1.01 $\pm$ 0.19 [0.47 - 1.61]  & 1.07 $\pm$ 0.19 [0.51 - 2.10] & 1.06 $\pm$ 0.18 [0.53 - 1.97]  & 1.00 $\pm$ 0.16 [0.66 - 1.56]  & 1.06 $\pm$ 0.18 [0.53 - 1.97]  & 0.98 $\pm$ 0.19 [0.66 - 1.34] & 1.07 $\pm$ 0.18 [0.49 - 1.99] & 1.07 $\pm$ 0.18 [0.49 - 1.99]  & 1.00 $\pm$ 0.20 [0.62 - 1.61]  \\
		    
		    Avg. TBS & 1.23 $\pm$ 0.13 [0.65 - 1.73] & 1.23 $\pm$ 0.13 [0.65 - 1.57]  & 1.19 $\pm$ 0.13 [0.79 - 1.73]  &  1.23 $\pm$ 0.13 [0.66 - 1.57] & 1.24 $\pm$ 0.12 [0.67 - 1.57]  & 1.20 $\pm$ 0.12 [0.79 - 1.46]  & 1.23 $\pm$ 0.13 [0.66 - 1.57]  & 1.17 $\pm$ 0.13 [0.79 - 1.39]    & 1.24 $\pm$ 0.12 [0.65 - 1.57] & 1.24 $\pm$ 0.12 [0.65 - 1.57]  & 1.19 $\pm$ 0.12 [0.79 - 1.42]    \\
		    \frax [\%] & 4.14 $\pm$ 4.39 [0.30 - 51.00] & 3.14 $\pm$ 3.07 [0.30 - 39.60]  & 7.04 $\pm$ 5.67 [0.90 - 44.50]  & 4.01 $\pm$ 4.28 [0.30 - 51.00] & 3.04 $\pm$ 2.93 [0.30 - 33.10]  & 6.29 $\pm$ 5.85 [0.90 - 44.50]  & 3.61 $\pm$ 3.74 [0.30 - 51.00]  & 8.53 $\pm$ 7.97 [1.40 - 44.50]  & 3.54 $\pm$ 3.56 [0.30 - 51.00] & 3.07 $\pm$ 2.89 [0.30 - 33.10]  & 5.76 $\pm$ 4.87 [0.90 - 30.20]   \\
		    \frax (w. aBMD)  [\%] &  4.45 $\pm$ 5.54 [0.00 - 51.00] & 3.38 $\pm$ 4.04 [0.00 - 51.00]  & 10.86 $\pm$ 9.09 [0.70 - 51.00] & 4.33 $\pm$ 5.41 [0.00 - 51.00] & 3.35 $\pm$ 3.95 [0.00 - 41.90]  & 10.47 $\pm$ 8.92 [0.70 - 51.00]  &   3.92 $\pm$ 4.83 [0.00 - 51.00]  & 14.38 $\pm$ 9.41 [2.80 - 41.60] & 3.85 $\pm$ 4.74 [0.00 - 51.00] & 3.34 $\pm$ 3.95 [0.00 - 51.00]  & 9.41 $\pm$ 8.56 [0.70 - 51.00]     \\
		    
		    \midrule
			
	        Training & - & - & - & - & 3403 & 128 & 3478 & 53 & - & 4353 & 107 \\
	        Validation & - & - & - & - & 790 & 27 & 810 & 7 & - &  1086 & 35 \\
			
		\end{tabular}
	}


	
\end{table}
}

\newcommand{\tblHorExtended}{
\begin{table}[tb]
		\caption{
		Extended results on CTN data and with 5 year horizon
	}
	\label{tbl:results}
%	\begin{subtable}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{l c c c c c  c  c c c }
			& & \multicolumn{5}{c}{Opportunistic Setting} & \multicolumn{3}{c}{Non-Opportunistic Setting}\\
			\cmidrule(r){3-7} \cmidrule(r){8-10}
			 &  & Base & Multiple & \makecell{GAP\\(CTN / CT / X-Ray)}  & \makecell{GAP + Base\\(CTN / CT / X-Ray)} & \makecell{GAP + Multiple\\(CTN / CT / X-Ray)} & \frax$^\dagger$ &  \makecell{aBMD +\\Base} & \makecell{\frax +\\Base} & \makecell{TBS +\\Base} & \frax + aBMD$^\dagger$\\
			
		    & \\
			
			&   & \makecell{60.89 $\pm$\\0.73} & \makecell{61.86 $\pm$\\0.88} & \makecell{80.87 $\pm$ 0.13/\\82.58 $\pm$ 0.21/\\77.24 $\pm$ 0.30} & \makecell{81.04 $\pm$ 0.17/\\ 82.48 $\pm$ 0.24/\\77.81 $\pm$ 0.38}  & \makecell{81.66 $\pm$ 0.23/\\82.52 $\pm$ 0.28/\\78.41 $\pm$ 0.33} & \makecell{68.49 $\pm$\\0.71} & \makecell{77.28 $\pm$\\0.58} & \makecell{60.50 $\pm$\\0.90} \\ 
			
				\midrule
			
			\makecell{CTN +\\Multiple}  & \makecell{81.66\\$\pm$ 0.23} &  \textbf{+20.77}&  \textbf{+19.80}&  \textbf{+0.78}/\textbf{-0.92}/\textbf{+4.41}  &  \textit{+0.61}/\textit{-0.82}/\textbf{+3.85}   &  - /\textit{-0.86}/\textbf{+3.24}  &  \textbf{+13.16}&  \textbf{+4.38} &  \textbf{+21.16}\\ 
            \makecell{CT +\\Multiple} & \makecell{82.52\\$\pm$ 0.28} &  \textbf{+21.63} &  \textbf{+20.66}&  \textbf{+1.64}/-0.06/\textbf{+5.28} &  \textbf{+1.47}/ +0.04/\textbf{+4.71}  &  \textit{+0.86}/ - /\textbf{+4.10}   &   \textbf{+14.03}&  \textbf{+5.24} &  \textbf{+22.02}\\ 
            \makecell{X-Ray +\\Multiple} & \makecell{78.41\\$\pm$ 0.33} & \textbf{+17.53} & \textbf{+16.56} & \textbf{-2.46}/\textbf{-4.17}/ \textit{+1.17} & \textbf{-2.63}/\textbf{-4.07}/ +0.61 & \textbf{-3.24}/\textbf{-4.10}/ - & \textbf{+9.92} & +1.14 & \textbf{+17.91}
			
	
			
		\end{tabular}
	}
	\subcaption{10 year hip fracture risk}
%	\end{subtable}
	%\begin{subtable}
	
	\resizebox{\textwidth}{!}{
		\begin{tabular}{l c  c c c c c  c c c }
			 & & \multicolumn{5}{c}{Opportunistic Setting} & \multicolumn{3}{c}{Non-Opportunistic Setting}\\
			\cmidrule(r){3-7} \cmidrule(r){8-10}
			 &  & Base & Full & \makecell{GAP\\(CTN / CT)}  & \makecell{GAP + Base\\(CTN / CT)} & \makecell{GAP + Full\\(CTN / CT)} & \makecell{aBMD +\\Multiple} & \makecell{\frax +\\Multiple} & \makecell{TBS +\\Multiple}\\
			
		    & \\
			
			&   & 64.88 $\pm$ 0.80 & 63.46 $\pm$ 1.12 & \makecell{88.49 $\pm$ 0.32/\\95.65 $\pm$ 0.27} & \makecell{89.35 $\pm$ 0.35/\\95.65 $\pm$ 0.37} & \makecell{89.62 $\pm$ 0.36/\\95.55 $\pm$ 0.30} &  71.63 $\pm$ 0.77 & 79.86 $\pm$ 0.86 & 61.76 $\pm$ 0.94 &\\ 
			
			\midrule 
			
			
 \makecell{CTN +\\Multiple}   & \makecell{89.62\\$\pm$ 0.36} &  \textbf{+24.73}&  \textbf{+26.16}&  +1.13/\textbf{-6.03}  &  +0.26/\textbf{-6.04}   &  - /\textbf{-5.93}  &  \textbf{+17.99}&  \textbf{+9.76} &  \textbf{+27.86}\\ 
 \makecell{CT +\\Multiple}   & \makecell{95.55\\$\pm$ 0.30} &  \textbf{+30.66}&  \textbf{+32.09}&  \textbf{+7.06}/-0.10 &  \textbf{+6.20}/-0.11  &  \textbf{+5.93}/ - &   \textbf{+23.92}&  \textbf{+15.69}& \textbf{ +33.79}\\ 
			
	
			
		\end{tabular}
	}
	
	\subcaption{5 year hip fracture risk}
}


\newcommand{\tblHor}{
\begin{table}[tb]
		\caption{
		Comparison fracture risk prediction --
		columns: different inputs which were used to train FORM;
		rows: different cohorts.
		All scores are given as mean val AUC $\pm$ SE. 
		Significant differences between the first and the other columns are marked italic (p $<$ 0.05) or bold  (p $<$ 0.01).
		$\dagger$ input not used for FORM
	}
	\label{tbl:results}
%	\begin{subtable}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{l c | c c c c | c c  }
			 Cohort & GAP + Multiple  &  Base & Multiple & GAP  & GAP + Base & \frax$\dagger$ \\

			
				\midrule
			
\makecell{X-Ray } & 78.41 $\pm$ 0.33  & \textbf{66.38 $\pm$ 1.76} & \textbf{69.67 $\pm$ 0.99} & \textit{77.24 $\pm$ 0.30} & 77.81 $\pm$ 0.38 &  77.43\\
            \makecell{CT } & 82.67 $\pm$ 0.21 &  \textbf{60.89 $\pm$ 0.73} &  \textbf{67.03 $\pm$ 0.93}&  82.58 $\pm$ 0.21 &  82.48 $\pm$ 0.24  &   75.94 \\
            
			
	
			
		\end{tabular}
	}
	
	\subcaption{Non-densitometric Settings}
	
		\resizebox{\textwidth}{!}{
		\begin{tabular}{l c |c c c | c c c c c c c}
			 Cohort & GAP + Multiple & \makecell{aBMD + Base} & \makecell{\frax + aBMD + Base} & \makecell{TBS + Base} & \frax + aBMD$\dagger$\\
			
	
			
				\midrule
			
 \makecell{X-Ray} & 78.41 $\pm$ 0.33  & \textbf{76.55 $\pm$ 0.89} & \textbf{81.50 $\pm$ 0.83} & \textbf{72.66 $\pm$ 1.34} & 80.92\\
            \makecell{CT} & 82.67 $\pm$ 0.21 &   \textbf{71.82 $\pm$ 0.50} &  \textbf{81.08 $\pm$ 0.34} &  \textbf{71.56 $\pm$ 0.39} &  79.19\\ 
           
			
	
			
		\end{tabular}
	}
	
	\subcaption{Densitometric Settings}

	
\end{table}
}

\newcommand{\tblCross}{
\begin{table}[tb]
		\caption{
		Cross-validation results (mean val. AUC $\pm$ STD) --
		columns: different methods / inputs;
		rows: cohort. Bold: results within a one percent margin of the best for each cohort.
	}
	\label{tbl:cross}
%	\begin{subtable}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{l c  c c c c c c c  }
	 &  \multicolumn{3}{c}{FORM} & \multicolumn{3}{c}{Cox} &  \frax  \\ %$\dagger$
	 \cmidrule(r){2-4} \cmidrule(r){5-7}
			 Cohort & GAP  & GAP + Base &  GAP + Multiple & GAP  & GAP + Base &  GAP + Multiple  & \\
			
			
				\midrule
			
			\makecell{X-Ray } & \textbf{81.57 $\pm$ 3.13} & \textbf{81.09 $\pm$ 3.18} & \textbf{81.44 $\pm$ 3.11} & 61.14 $\pm$ 16.80 & 70.26 $\pm$ 5.71 & 70.19 $\pm$ 6.58  &  74.72 $\pm$ 7.21 \\

            \makecell{CT } & 77.53 $\pm$ 5.81 &  \textbf{80.66 $\pm$ 3.75}  &  \textbf{81.04 $\pm$ 5.54} & 67.56 $\pm$ 23.97 & 73.69 $\pm$ 9.22 & 75.35 $\pm$ 9.11 &   74.74 $\pm$ 5.70\\
             
			
			
			\midrule
			
	
			
		\end{tabular}
	}
	

	
\end{table}
}

\newcommand{\tblRiskFactors}{
\begin{table}[tbh]
		\caption{
	 Overview about individual elements of the risk factor groups
	}
	\label{tbl:risk}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{l l }
		
		Risk factor group & Individual Elements \\
		
		\midrule
		Base & age, BMI, height, fat mass, clinic \\
		Multiple  &  \makecell[l]{Base +  previous fractures spine/hip, osteoporosis in parents,  fall history, professional background,\\
		previous diseases like cancer or hypertension  and smoking and alcohol habits} \\
		aBMD  & spinal and femoral aBMD \\
		\frax & \frax 10 year risk  for hip and major osteoporotic fracture with and without usage of aBMD \\
		TBS & Average TBS across spine \\
		
		\end{tabular}
	}
\end{table}
}

\newcommand{\tblAblation}{
\begin{table}[thb]
		\caption{
	 Ablation of hyperparameters on CTN data for 10 and 5 year hip fracture risk --
	 Significant differences to the baseline are marked italic  (p $<$ 0.05) or bold  (p $<$ 0.01).
	}
	\resizebox{\textwidth}{!}{
		\begin{tabular}{l c  c c c c c  c c c }
			& \multicolumn{3}{c}{10 year risk} & \multicolumn{3}{c}{5 year risk}\\
			\cmidrule(r){2-4} \cmidrule(r){5-7}
			
			&  GAP & GAP + Base & GAP + Multiple  &  GAP & GAP + Base & GAP + Multiple \\
			 
			CTN & 80.87 $\pm$ 0.13 & 81.04 $\pm$ 0.17 & 81.66 $\pm$ 0.23 & 88.49 $\pm$ 0.32 & 89.35 $\pm$ 0.35 & 89.62 $\pm$ 0.36 \\ 
			\midrule
	%		CT & 82.58 $\pm$ 0.21 & 82.48 $\pm$ 0.24 & 82.67 $\pm$ 0.21 &  95.65 $\pm$ 0.27 & 95.65 $\pm$ 0.37 & 95.55 $\pm$ 0.30\\
 Dropout rate 0.4 &   \textit{-0.34} (80.53 $\pm$ 0.18)&  -0.18 (80.87 $\pm$ 0.27)&  \textit{-0.98} (80.68 $\pm$ 0.33)	&   -0.47 (88.01 $\pm$ 0.37)&  -1.14 (88.21 $\pm$ 0.43)&  \textit{-2.00} (87.61 $\pm$ 0.44)\\ 
 Min-Max-Normalization   &   +0.05 (80.92 $\pm$ 0.19)&  -0.04 (81.00 $\pm$ 0.17)&  \textit{-0.65} (81.00 $\pm$ 0.25) &   -0.15 (88.34 $\pm$ 0.43)&  -0.99 (88.37 $\pm$ 0.37)&  -1.21 (88.41 $\pm$ 0.54)\\ 
 Smaller MLP &   -0.40 (80.47 $\pm$ 0.40)&  -0.13 (80.92 $\pm$ 0.24)&  \textit{-0.70} (80.95 $\pm$ 0.25) & +0.05 (88.54 $\pm$ 0.53)&  -0.24 (89.12 $\pm$ 0.52)&  -1.91 (87.70 $\pm$ 0.58)\\ 
 Larger MLP &   -0.02 (80.86 $\pm$ 0.14)&  \textbf{+0.57} (81.61 $\pm$ 0.21)&  -0.20 (81.46 $\pm$ 0.31)&   +0.42 (88.91 $\pm$ 0.28)&  \textbf{-1.83} (87.52 $\pm$ 0.25)&  \textbf{-2.32} (87.30 $\pm$ 0.32)\\  
No input merging  &   +0.01 (80.88 $\pm$ 0.22)&  -0.19 (80.86 $\pm$ 0.19)&  \textbf{-0.78} (80.87 $\pm$ 0.19)&   +0.72 (89.21 $\pm$ 0.41)&  \textit{-1.60} (87.75 $\pm$ 0.31)&  \textbf{-3.04} (86.58 $\pm$ 0.28) \\
Input merging with s = 1  &   -0.40 (80.47 $\pm$ 0.28)&  +0.10 (81.15 $\pm$ 0.25)&  -0.32 (81.34 $\pm$ 0.29)&   +0.12 (88.61 $\pm$ 0.39)&  \textit{-1.83} (87.52 $\pm$ 0.45)&  -1.90 (87.72 $\pm$ 0.51)  
			
		\end{tabular}
	}
	\label{tbl:ablation}
\end{table}
}

\newcommand{\tblDatasets}{
\begin{table}[thb]
		\caption{
	 Overview of reason for exclusion of patients -- We start for all cohorts with the total study population. The reasons for certain exclusions and number of excluded cases are given in white rows and the left over people are given in the grey rows.
	}
	\resizebox{\textwidth}{!}{
	\begin{tabular}{c c c c  c c c c c  c c c }
			& \multicolumn{3}{c}{Cohort All} & \multicolumn{5}{c}{Cohort CT} & \multicolumn{3}{c}{Cohort X-Ray}\\
			\cmidrule(r){2-4} \cmidrule(r){5-9} \cmidrule{10-12}
			
			& & \multicolumn{2}{c}{$t$ = 10 year} & & \multicolumn{2}{c}{$t$ = 10 year} & \multicolumn{2}{c}{$t$ = 5 year} & & \multicolumn{2}{c}{$t$ = 10 year} \\
			\cmidrule(r){3-4} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule{11-12}
			
			& all & w/o fx & w fx & all & w/o fx & w fx  & w/o fx & w fx & all & w/o fx & w fx \\
			
			\rowcolor{LightGray}
			
			Start & 5994 & 5994 & 5994 & 5994 & 5994 & 5994 & 5994 & 5994 & 5994 & 5994 & 5994 \\
			
			\makecell{Not all risk\\factors present} & N/A & N/A & N/A & 52 & 52 & 52 & 52 & 52 & 52 & 52 & 52  \\
			\rowcolor{LightGray}
			& 5994 & 5994 & 5994 & 5942 & 5942 & 5942 & 5942 & 5942 & 5942 & 5942 & 5942   \\
			
			\makecell{No Image\\Data} & N/A & N/A & N/A & 2670 & 2670 & 2670 & 2670 &  2670 & 1759 & 1759 & 1759\\
			\rowcolor{LightGray}
			& 5994 & 5994 & 5994 & 3272 & 3272 & 3272 & 3272 & 3272 & 4183 & 4183 & 4183  \\
			
			\makecell{Censored} & N/A & 1805 & 1805 & N/A & 970 & 970 & 970 & 970 & N/A & 762 & 762 \\
			\rowcolor{LightGray}
			& 5994 & 4189 & 4189 & 3272 & 2302 & 2302 & 2302 & 2302 & 4183 & 3421 & 3421\\
			
			\makecell{Both Hips\\not usable} & N/A  & N/A & N/A & 107 & 72 & 72 & 72 & 72 & 288 & 224 & 224   \\
			\rowcolor{LightGray}
			& 5994 & 4189 & 4189 & 3165 & 2230 & 2230 &  2230 & 2230 & 3895 & 3197 & 3197 \\
			
			Wrong Class & N/A & 185 & 4004 & N/A & 80 & 2150 & 32 & 2198 & N/A & 89 & 3108  \\
			\rowcolor{LightGray}
		    $n$ & 5994 & 4004 & 185 & 3165 & 2150 & 80 & 2198 & 32 & 3895 & 3108 & 89 \\


			
		\end{tabular}
	}
	\label{tbl:datasets}
\end{table}
}

